Tag Embedding Based Personalized Point Of Interest Recommendation System

Personalized Point of Interest recommendation is very helpful for satisfying users' needs at new places. In this article, we propose a tag embedding based method for Personalized Recommendation of Point Of Interest. We model the relationship between tags corresponding to Point Of Interest. The model provides representative embedding corresponds to a tag in a way that related tags will be closer. We model Point of Interest-based on tag embedding and also model the users (user profile) based on the Point Of Interest rated by them. finally, we rank the user's candidate Point Of Interest based on cosine similarity between user's embedding and Point of Interest's embedding. Further, we find the parameters required to model user by discrete optimizing over different measures (like ndcg@5, MRR, ...). We also analyze the result while considering the same parameters for all users and individual parameters for each user. Along with it we also analyze the effect on the result while changing the dataset to model the relationship between tags. Our method also minimizes the privacy leak issue. We used TREC Contextual Suggestion 2016 Phase 2 dataset and have significant improvement over all the measures on the state of the art method. It improves ndcg@5 by 12.8%, p@5 by 4.3%, and MRR by 7.8%, which shows the effectiveness of the method.

==> contextual-ipm published/introduction.tex <==
\section{Introduction}
\label{sec:intro}
Recent times have seen a growing interest in \emph{proactive} Information
Retrieval (IR) systems~\cite{DBLP:conf/ecir/BhatiaMA16} and related ideas
such as contextual suggestions~\cite{hashemi2016overview}, and zero-query
search systems. Such systems are designed to provide information that is
helpful to a user, given her current circumstances, without requiring the
user to submit an explicit query. Recommender Systems (RSs) that suggest
potentially interesting tourist attractions --- or \emph{Points Of
  Interest} (POIs) --- to travellers are examples of such proactive
systems. POI recommender systems~\cite{borras2014intelligent} seek to
address the following scenario. A tourist, while on a trip to a certain
place, looks for interesting things to do and sites to visit. The system
considers the traveller's current location and other factors (e.g., the
weather, whether the user is alone or with a group of friends). Based on its
prior knowledge about her preferences, it then recommends local POIs that
are most likely to be of interest to her.

The TREC Contextual Suggestion Track (TCST) that ran during
2012 -- 2016~\cite{DBLP:conf/trec/Dean-HallCKTV12,DBLP:conf/trec/Dean-HallCSKTV13,DBLP:conf/trec/Dean-HallCKTV14,DBLP:conf/trec/Dean-HallCKKV15,DBLP:conf/trec/HashemiKKCV16}
provided a comprehensive framework for investigating and evaluating RSs for
POIs. As with many other TREC tracks, the data and task definition for this
track evolved during its lifetime. In its final year (2016), an important
new feature was introduced: each POI was annotated with
user-assigned \emph{tags}\footnote{These were also called
  \emph{endorsements} at TREC.}. Tags are short descriptive labels assigned
to POIs by end-users. For example, the POI \emph{The Fitzwilliam Museum}\footnote{\url{https://www.fitzmuseum.cam.ac.uk/}} might be annotated
with the tags \ptag{museum} and \ptag{history}; similarly, \emph{Keen’s Steakhouse}\footnote{\url{http://www.keens.com/}}
could be tagged with \ptag{restaurant} and \ptag{pub}. More generally, the
use of tags has become a widespread practice in social media as a means of
quickly describing or classifying various items, like blog posts,
photographs, audio/video clips, etc. Hashtags in microblog posts are
possibly the most commonly encountered form of user-assigned tags.
Figure~\ref{fig:tweet1} shows an anonymous tweet describing an outing. The
tags assigned by the user to this tweet provide information about the
\emph{trip~type} (\ptag{nightout, dinner}), as well as the accompanying
\emph{type~of~group} ({\ptag{friends}}).
%
\begin{figure}
  \centering
  \includegraphics[scale=0.3]{figs/tweet1.jpg}
  \caption{A sample tweet (anonymous) where the hashtags are indicative of the basic information contained in the tweet.}
  \label{fig:tweet1}
\end{figure}
%
It is clear that user-assigned tags provide various types of information
(e.g., the \emph{category} of a POI --- \ptag{restaurant}, \ptag{museum})
that would be useful in the context of recommending POIs. Intuition
suggests that it should be possible to utilize this additional information
to provide better recommendations. Indeed, ``participants [at the TCST,
2016] showed considerable interest in using endorsements to improve
their contextual suggestion systems''~\cite{DBLP:conf/trec/HashemiKKCV16}.
In this study, we propose a method that leverages tags to improve the
quality of recommendations. Experimental results on the TCST 2016 data
suggest that the proposed method significantly advances the state of the
art.

Our proposed approach is primarily content-based. That is, if a
person % $X$
has rated POIs $h_1, h_2, \ldots, h_m$ highly, but has given a low rating
to $l_1, l_2, \ensuremath{\ldots}, l_n$, then the predicted rating for POI
$p$ would depend on whether $p$ is more similar to $h_1, h_2, \ldots, h_m$
or to $l_1, l_2, \ensuremath{\ldots}, l_n$. From an IR perspective, one
natural way to quantify the similarity between two POIs would be to compute
the overlap between their textual descriptions. As indicated above, we
simply consider the set of tags assigned to a POI as its textual
description.
% \footnote{Alternative definitions of textual descriptions are discussed in Section~\ref{sec:conclusion}.} 
If we consider an operational
system (e.g., a mobile app) that actually implements our proposed method,
its interface could be designed to make it easy for an end-user to assign
tags to POIs. On the one hand, user-assigned tags are expected to be
high-quality content descriptors, somewhat analogous to keywords assigned
by subject experts. On the other hand, the number of tags assigned to a POI
will typically be small: for the TCST 2016 data, each POI was assigned 2.73
tags on an average. Thus, for this representation, the well-known
\emph{vocabulary mismatch problem}, which plagues any bag-of-words based
representation, is expected to be even more severe.
% different people may use different words while describing the same
% concept; thus, there may exist only a weak overlap between the BOWs of
% two texts that are semantically strongly related.

Word embeddings~\cite{mikolov2013distributed,pennington2014glove}
constitute a modern approach to tackling this problem. Broadly, an
embedding technique uses word-cooccurrence statistics from a (preferably large)
corpus of unlabelled textual data to map each word to a vector in a
low-dimensional, abstract space (the so-called \emph{embedding} space) in
such a way that the similarity between the vectors reflects the semantic
relationship between the corresponding words. Further, some simple vector
operations in the embedding space (e.g., addition and subtraction)
correspond nicely to linguistic notions such as conceptual combination, and
analogies. Embedding techniques have proven to be very useful in various
text processing tasks.

If embeddings are appropriately generated for POI tags, we expect that the
embeddings of `art galleries', `museums', and `poetry readings' will be
relatively close to each other, but relatively distant from the embeddings
of `parks', and `hiking trails'. Our approach, based on this intuition, can
be summarized as follows.
\begin{enumerate}
\item Embeddings are generated for all tags assigned to POIs.
\item For a particular POI, the embeddings of tags assigned to it are
  aggregated to obtain a representation of the POI in the embedding space.
\item Using Rocchio's algorithm~\cite{rocchio1971relevance} with the
  positive, negative and neutral ratings assigned by a traveller to various
  POIs, a profile is created for that traveller. This profile, also a
  vector in the embedding space, is expected to constitute an abstract, but
  high-level, description of the traveller's `type': whether the user prefers
  outdoor activities, or inclined towards the arts and
  literature, or whether of `food-drink-party' type, etc.
\item The profile of a traveller is matched against the vector
  representations of potential POIs, to be recommended, to assign scores. 
  Based on the scores, a ranked list of POIs are to be suggested to the user.
%\item Finally, the ranked list created above is refined using a filter (or a binary classifier) 
% to create a ranked list of suggested POIs. 
\end{enumerate}
% \textbf{\textcolor{red}{M: CHECK}}
Note that, in order to generate the embeddings in Step 1 above, we consider
the tags assigned by \emph{all} users to various POIs. 
% This gives our
% approach a slight flavour of collaborative filtering, in the sense that we
% need access to a full user-item matrix. Note, however, that user 
% ratings are not made use of, only descriptions.

In the next section, we summarize the contributions of this work.
Section~\ref{sec:related-work} discusses related work and
Section~\ref{sec:terminology} provides a quick review of the terminology
used in the TCST. The proposed method is described in detail in
Section~\ref{sec:approach}. Experimental results are presented and
discussed in Sections~\ref{sec:results} and \ref{sec:discussion}.
The article concluded in Section~\ref{sec:conclusion} listing an issue
that needs further investigation.

%In this work, we have used tags to model users in order to perform POI recommendation. We can divide our approach into four steps:
%\begin{itemize}
%\item Step I: We model the relationship between tags using word embedding.
%\item Step II: We use tag embedding to obtain vector representation of user profile, POIs.
%\item Step III: We generate a score to rank candidate Point Of Interest using cosine similarity between user profile representation vector and POI representation vector.
%\item Step IV: Further we can refine ranking using binary classification, which classifies the relevance of a Point Of Interest with context.
%\end{itemize}
%In this work, we also find the parameter in the search space using optimization instead of choosing it heuristically.

%All of the generated data is sensitive and personal to the user, which could reveal his identity. As all of the data is processed on the system site the privacy is compromised. To maintain the privacy of sensitive data is another challenge~\cite{barkhuus2003location, knijnenburg2013making}. 

%Shifted to related work. 
%A new research domain, called \emph{TREC Contextual Suggestion} track\footnote{\url{https://trec.nist.gov/data/context.html}} was started in TREC~2012 %considering this particular research question. 
%The broad
%objective underlying the track was the study of techniques for addressing
%``complex information needs that are highly dependent on context and user
%interests''~\cite{hashemi2016overview,DBLP:conf/trec/Dean-HallCKKV15,DBLP:conf/trec/Dean-HallCKTV14,DBLP:conf/trec/Dean-HallCSKTV13,DBLP:conf/trec/Dean-HallCKTV12}.

% \subsection{Problem statement}
% \label{sec:problem-statement}
% Assume a traveller in a specific context (e.g., a city and trip type) is seeking things to do that reflect their own interests, which is supposed to be inferred from their interests in the given context and a visited city.
% User's profile has Point Of Interest list with their tags/endorsements, and ratings from the cities visited by him. We need to make recommendations for attractions in a new context (including the target city as the location) using his profile information.
%We also tried to resolve the privacy issue by utilizing the computation power and storage of smart devices. We could store the personal info at the user's device end and generate the user profile using its computation power.
% \subsection{Overview of approach}
% \label{sec:overview}

\section{Our Research Contribution} \label{sec:contrib}
\para{Research Objective}
Researches on venue recommendation surged its popularity among practitioners with the emerging usage of services like Foursquare, Tripadvisor, Yelp etc. across the globe.
The development of a productive recommender system would indeed be supportive to the users of services like these.
% is a step towards a smarter contextualized search system that would be able to appropriately suggest places to visit, or activities to the users and would be a steep jump towards the development of a `zero query search' system.
% With the emerging popularity of services like Yelp, Tripadvisor, etc., research on venue recommendation surged its popularity among researchers.
% The purpose of this study is to build a recommender system based on one's preferences.
In this study, we propose to build a POI recommender system that would suggest places to visit considering the preferences of the user.

\para{Theoretical Contribution}
Given a fairly sized text collection containing well-formed sentences, word embedding techniques can produce a low-dimensional representation of words capturing the semantic relatedness of the terms.
The application of word embedding techniques for different text processing tasks have shown the effectiveness of the methods in terms of improving performances.
% In this article, we discuss that word embedding
% Word embedding techniques have shown their proficiency in capturing semantic regularities on the basis of word co-occurrence in fairly sized text corpora.
% The improvements, when applied for various text classification tasks, have been remarkable.
In this study, we argue that embeddings, when trained using a dataset consisting of informal tags without proper sentence structure, can also adept at capturing term relatedness. % similar to the scenario when the embeddings are trained using a fairly sized text dump.

\para{Practical Implication}
The practical implication of the presented work lies in the empirical examination on whether training an embedding model using informal texts with casual labels could in effect capture the semantic regularities.
Experimentation on TREC Contextual Suggestion Track data
% and comparison with some of the best performing systems, 
validates the significant predominance of the proposed embedding based approach over state-of-the-art techniques on the benchmark dataset.
Possible risk of most recommender systems is the concern of privacy breach that may happen due to the sharing of personal preferences with the server.
With this respect, the proposed approach is secure as the method can be designed to employ the user preferences for suggestions solely on the client's side without getting exposed to the server-side endpoint.
% The relatively less information of users getting exposed to the endpoint (server-side) makes the approach more secure as well.
% Further, we suggested a way to tune the parameters using discrete optimization instead of choosing it heuristically or using cross validation, Along with it shows the variation of result on changing measures to tune the parameters.
% Tags based Recommendation, which is effective and required less info from user, as it is easier for user to tag place then write whole comment. 
% Much little info of user is being exposed to the end point(server side). 
% Significant improvement over existing state of the art in all measures. 
% Shows the importance of Tags and its relationship in POI recommendation system, since all the naive work leads to significant improvement. 
All codes and data that has been used in this article are available for reproducibility and further research purposes\footnote{\url{https://github.com/sagrawal1993/ContextualSuggestion}}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "contextual-suggestions"
%%% End:

